Massively Multilingual Adversarial Speech Recognition

We report on adaptation of multilingual end-to-end speech recognition models trained on as many as 100 languages. Our findings shed light on the relative importance of similarity between the target and pretraining languages along the dimensions of phonetics, phonology, language family, geographical location, and orthography. In this context, experiments demonstrate the effectiveness of two additional pretraining objectives in encouraging language-independent encoder representations: a context-independent phoneme objective paired with a language-adversarial classification objective.

==> ablation.tex <==
\begin{figure}
\centering
\begin{tikzpicture}
\begin{axis}[
    %scaled x ticks = true,
        %grid style=dashed,
%       width=4.55cm,
%        height=4.5cm,
        yticklabel style={
                /pgf/number format/fixed,
                /pgf/number format/precision=1,
                /pgf/number format/fixed zerofill
        },
        xticklabel style={
                /pgf/number format/fixed,
                /pgf/number format/precision=0,
                /pgf/number format/fixed zerofill
        },
        ylabel={Word error rate (\%)},
        xlabel={Utterances (will change to minutes)},
%       title={Geometric prior},
        %legend pos = north west,
        legend columns=4,
%        legend entries={None;, CLWE;, OTS-Duong;, GNC},
        legend to name=named,
%        xtick={1000, 2000, 4000, 8000, 16000, 32000, 64000, 128000},
        xmode=log,
        log ticks with fixed point
        ]

\addplot[black, legend entry=mlg, mark=x]
% gensim_w2v.en.ws353sents.d200.w48.cbow0 (ie. Skip-gram)
coordinates {
     (125, 96.5)
     (250, 98.0)
     (500, 88.5)
     (1000, 84.8)
     (2000, 77.5)
     (4000, 70.6)
     (8992, 66.6)
};
\addplot[black, dashed, legend entry=mlg+phn+adv, mark=x]
% gensim_w2v.en.ws353sents.d200.w48.cbow0 (ie. Skip-gram)
coordinates {
     (125, 99.7)
     (250, 92.5)
     (500, 87.2)
     (1000, 78.4)
     (2000, 75.8)
     (4000, 71.2)
     (8992, 68.3)
};

\addplot[blue, legend entry=kia, mark=x]
% gensim_w2v.en.ws353sents.d200.w48.cbow0 (ie. Skip-gram)
coordinates {
     					
     (125, 70.1)
     (250, 65.2)
     (500, 61.7)
     (1000, 58.1)
     (2000, 55.2)
     (4000, 52.9)
     (8992, 51.9)
};

\addplot[blue, dashed, legend entry=kia+phn+adv, mark=x]
% gensim_w2v.en.ws353sents.d200.w48.cbow0 (ie. Skip-gram)
coordinates {
     (125, 68.7)
     (250, 64.8)
     (500, 59.9)
     (1000, 56.4)
     (2000, 54.7)
     (4000, 53.7)
     (8992, 51.5)
};

\end{axis}
\end{tikzpicture}\\
\ref{named}
\caption{Malagasy adaptation on the non-evaluation speaker. The auxiliary objectives facilitate a better initialization, but the advantage is lost as mismatch between adaptation and evaluation speakers becomes the most dominant factor. Should add more langs here.}
\label{fig:ablation}
\vspace{-3mm}
\end{figure}

==> swedish_scaling.tex <==
\begin{figure}
\centering
\begin{tikzpicture}
\begin{axis}[
    %scaled x ticks = true,
        %grid style=dashed,
%       width=4.55cm,
%        height=4.5cm,
        yticklabel style={
                /pgf/number format/fixed,
                /pgf/number format/precision=1,
                /pgf/number format/fixed zerofill
        },
        xticklabel style={
                /pgf/number format/fixed,
                /pgf/number format/precision=0,
                /pgf/number format/fixed zerofill
        },
        ylabel={Word error rate (\%)},
        xlabel={Utterances (will change to minutes)},
%       title={Geometric prior},
        %legend pos = north west,
        legend columns=4,
%        legend entries={None;, CLWE;, OTS-Duong;, GNC},
        legend to name=named,
%        xtick={1000, 2000, 4000, 8000, 16000, 32000, 64000, 128000},
        xmode=log,
        log ticks with fixed point
        ]


\addplot[black, legend entry=vanilla, mark=x]
coordinates {
     					
     (125, 70.1)
     (250, 65.2)
     (500, 61.7)
     (1000, 58.1)
     (2000, 55.2)
     (4000, 52.9)
     (8992, 51.9)
};

\addplot[black, dashed, legend entry=+phn+adv, mark=x]
coordinates {
     (125, 68.7)
     (250, 64.8)
     (500, 59.9)
     (1000, 56.4)
     (2000, 54.7)
     (4000, 53.7)
     (8992, 51.5)
};

\end{axis}
\end{tikzpicture}\\
\ref{named}
\caption{Malagasy adaptation on the non-evaluation speaker. The auxiliary objectives facilitate a better initialization, but the advantage is lost as mismatch between adaptation and evaluation speakers becomes the most dominant factor. Should add more langs here.}
\label{fig:ablation}
\vspace{-3mm}
\end{figure}
